CORAL: Contextual Response Retrievability Loss Function for Training Dialog Generation Models

In the field of Natural Language Processing, there are many tasks that can be tackled effectively using the cross-entropy (CE) loss function. However, the task of dialog generation poses unique challenges for CE loss. This is because CE loss assumes that, for any given input, the only possible output is the one available as the ground truth in the training dataset. But, in dialog generation, there can be multiple valid responses (for a given context) that not only have different surface forms but can also be semantically different. Furthermore, CE loss computation for the dialog generation task does not take the input context into consideration and, hence, it grades the response irrespective of the context. To grade the generated response for qualities like relevance, engagingness, etc., the loss function should depend on both the context and the generated response. To address these limitations, this paper proposes CORAL, a novel loss function based on a reinforcement learning (RL) view of the dialog generation task with a reward function that estimates human preference for generated responses while considering both the context and the response. Furthermore, to overcome challenges such as high sample complexity of RL training and a large action space, we propose a mix-policy training algorithm. Notably, using CORAL we can train dialog generation models without assuming the ground-truth as the only correct response. Extensive comparisons on benchmark datasets demonstrate that CORAL based models outperform strong state-of-the-art baseline models of different sizes.

==> OLD/Front_Matter/Introduction.tex <==
\section{Introduction}
\label{intro}


% \textsc{\textbf{Theme}: From NLP for Text to NLP for Dialog Systems}
% 
% Dialog System tasks are often framed as other problems in NLP. But in this process of remapping the problems of dialog understanding or generation to well understood problems in NLP we often lose some of the essence / aspects of conversational texts.
% 
% ======================================
 
NLP for Dialog Systems intends to study and imitate the reasoning process behind human-human conversations. The long-term goal of this area of research is to build intelligent agents that can carry out successful conversations with humans. The task of conversation is considerably different from other NLP tasks (mainly the ones dealing with monologic text inputs) at a very fundamental level. To give a few examples, such differences are due to the presence of speech acts - \cite{austin1975speechacts}, dialogic pairs - \cite{harris2004adjpair,schegloff1968adjpair}, joint actions and grounding - \cite{stalnaker1978assertion}, implicature - \cite{grice1975logic}, etc. 

Because of this, when we try to model any response-generation task as simple Seq2Seq learning problems, we often ignore a lot of core aspects of the dialog process. It has not stopped researchers from training neural models \cite{adiwardana2020meenabot,roller2020blender,bao2020plato,zhang2019dialogpt}, often utilizing very large-scale data and computational resources. Some of these models may seem very good with a fleeting glance, but if we start to look deeply into the behavior of these models, many issues start to appear (for easy reference, we give some examples of such cases in Section \ref{sec:examples}, page \pageref{sec:examples}). Here we would like to point out a few traits of these approaches:

\begin{enumerate}
 \item Even to get these models to produce the most basic and sensible responses, ignoring the rest of the issues discussed below, one generally has to invest orders of magnitude more data and computational resources than any other ML/NLP problem. 
 \item We have absolutely no control over what these models generate once they have been trained/deployed. Compared to these, even the rule-based Mitsuku\footnote{https://www.pandorabots.com/mitsuku/} model is relatively more controllable in terms of what response it produces or what knowledge source it uses.
 \item These samples also highlight the possible insufficiency of the various evaluation metrics (both automatic and human evaluation based) in capturing the types of problems reported in examples of Section \ref{sec:examples} (Page \pageref{sec:examples}).
\end{enumerate} 
 
Based on these observations, we argue that we should make better design choices than directly applying architectures from other domains. We can incorporate various inductive biases for dialog model architectures based on the large body of literature on human-human conversations [CITE] from the last five decades. Motivated these shortcomings of commons model designs that perform very effectively in other NLP tasks but fails to generalize for training dialog systems, we ask the following research questions. [\textbf{RQ1}] \textit{How can we incorporate our prior knowledge about the structure and the underlying process supporting successful human-human conversations towards mitigating the problems faced by current approaches for dialog representation learning or generation?}

In Section \ref{sec:hier-main}, we investigate how the inductive bias of hierarchy can help improve the performance of transformer-based response generation models. Such hierarchy is inherently present in context inputs to any dialog system. This is the hierarchy that exists between the three semantic information units of any dialog context; these are words, utterances, and the overall context input. 

In all of Machine Learning, various evaluation metrics have been designed to compare competitive systems and determine where a particular system falls short. Current evaluation metrics used for dialog systems lack in this second property. To this end, we propose the second research question: [\textbf{RQ2}] \textit{Can we design evaluation metrics for dialog systems that evaluate specific and well-understood features of the generated response than the overall quality of the models?}

In the work described in Section \ref{sec:feateval-main}, we delve into the problem of designing evaluation metrics for assessing specific aspects of a generated dialog. More specifically, we identify that various utterance-level features follow specific patterns in human conversations. The presence of these patterns helps in effective communication between the speakers during a conversation.


==> OLD/Front_Matter/acknowledgement.tex <==
\newpage

{\hspace{5.5cm}\Large {\bf Acknowledgements}}
\newline

First and foremost, I take this opportunity to express my deepest regards to my supervisors {\em Dr. Pawan Goyal} and {\em Dr. Sourangshu Bhattacharya}, for their continuous support and guidance. Working with them continues to be an extremely knowledgeable experience. I would also like to thank the members of the \textbf{C}omplex \textbf{Ne}twork \textbf{R}esearch \textbf{G}roup (\textbf{CNeRG, IIT Kharagpur}) for their constant motivation and enlightenment through countless discussions. Finally, I express my gratitude towards {\em Prof. Niloy Ganguly} for believing in me when the times were rough and providing me with the required encouragement to continue with my PhD.

\vspace{0.5cm}

I would like to convey my regards to the {\em Department of Computer Science and Engineering} and all its staffs for allowing me to perform my research here. A sincere thanks to {\em Prof. Dipanwita Roychowdhury}, Head, Department of Computer Science and Engineering, for her continued supervision, encouragement and affection. I shall forever remain indebted to my family members, teachers and friends for supporting me at every stage of my life. It is their blessings, encouragement and support that keeps me going. Lastly, I would like to thank {\em Dr. Saptarshi Ghosh} for inspiring me with his work ethics, and his extremely approachable and comforting nature.

\vspace{1cm}
\noindent Department of Computer Science and Engineering, \\
IIT Kharagpur \\
2020. \\

\hfill (Rajdeep Mukherjee) 

==> OLD/Front_Matter/certificate.tex <==
\newpage

{\hspace{6cm}\Large {\bf Certificate}} \newline

This is to certify that the work presented in this report entitled ``Inductive Bias Motivated Solutions for Dialog Generation and Evaluation'', submitted by Bishal Santra, having examination roll number 18CS91R06, has been carried out under our supervision for the partial fulfillment of the  requirements for the degree of {\em Doctor of Philosophy
}in Computer Science and Engineering, in the Department of Computer Science and Engineering, IIT Kharagpur.

\vspace*{0.9cm}

\begin{flushleft}
	------------------------------------ \hfill ------------------------------------  \\
	Dr. Pawan Goyal  \hfill Dr. Sourangshu Bhattacharya \\ (Supervisor) \hfill (Joint supervisor)
	\hfill  \\
	%\linebreak
\end{flushleft}

\vspace{0.5cm}

\begin{flushleft}
	------------------------------------ \hfill ------------------------------------  \\
	Prof. Niloy Ganguly  \hfill Dr. Saptarshi Ghosh \\ (DSC Chairman) \hfill (DSC Member)
	\linebreak
\end{flushleft}

\begin{flushleft}
	------------------------------------ \hfill ------------------------------------  \\
	Dr. Animesh Mukherjee  \hfill Dr. Jiaul Hoque Paik \\
	(DSC Member) \hfill (DSC Member) 
	\linebreak
\end{flushleft}

\begin{flushleft}

	\hspace{5.2cm} --------------------------------------- \\ \hspace{5.25cm}
 	Prof. Dipanwita Roychowdhury \\ \hspace{5.5cm} (Head of Department, CSE)
\end{flushleft}

\vspace{4 cm}
\begin{flushright}
	---------------------- \\
	Date \enspace \enspace \enspace \enspace 
	
\end{flushright}


		

==> OLD/Front_Matter/publication.tex <==
\newpage
{\LARGE \textbf{Publications}} \newline \newline

{\Large {\bf Refereed Conferences} } %\newline %\newline
\begin{enumerate}
    \item \textbf{Rajdeep Mukherjee}, Shreyas Shetty, Subrata Chattopadhyay, Subhadeep Maji, Samik Datta and Pawan Goyal. \textit{Reproducibility, Replicability and Beyond: Assessing Production Readiness of Aspect Based Sentiment Analysis in the Wild}, Proceedings of the 43rd European Conference on Information Retrieval (ECIR'21), Virtual Event, Lucca, Italy
    \item \textbf{Rajdeep Mukherjee}, Hari Chandana Peruri, Uppada Vishnu, Pawan Goyal, Sourangshu Bhattacharya, Niloy Ganguly. \textit{Read what you need: Controllable Aspect-based Opinion Summarization of Tourist Reviews}, Proceedings of the 43rd International ACM SIGIR Conference on Research and Development in Information Retrieval (SIGIR'20), Virtual Event, China
\end{enumerate}

==> OLD/Front_Matter/synopsis-titlepage.tex <==
\thispagestyle{empty}
\begin{titlepage}
\begin{center}
    \vspace*{0.5in}
    {\huge\textbf{CORAL: Contextual Response Retrievability Loss Function for Training Dialog Generation Models}} \\
    \vspace{0.6in}
     {\large\bf Extension Seminar Report Submitted in Partial Fulfillment\\ of the Requirements for the Degree of }\\
     \vspace{0.3in}
     {\large\bf Doctor of Philosophy}\\
     {\large\bf in}\\
     {\large\bf Computer Science and Engineering}\\     
    \vspace{0.5in}
    {\large\bf by}\\
    \vspace{0.3in}
    {\Large\bf Bishal Santra}\\
    \vspace{0.1in}
    {\Large\bf Roll Number: 18CS91R06}\\
    \vspace{0.5in}
    {\large\bf Under the supervision of}\\
    \vspace{0.2in}
    {\Large\bf  Dr. Pawan Goyal}\\
     \vspace{0.1in}
    %  {\Large\bf and}\\
    %  \vspace{0.1in}
    %  {\Large\bf  Dr. Sourangshu Bhattacharya}\\
    
    \vspace{0.5in}
    \begin{center}
        \includegraphics[width=1.2in]{Front_Matter/figures/IIT_Kharagpur_Logo.png}
    \end{center}
    {\Large\textbf{Department of Computer Science and Engineering,}}\medskip\\
    {\Large\textbf{Indian Institute of Technology Kharagpur}}\medskip\\
    {\large\textbf{February 2022}}
\end{center}
\end{titlepage}

